Controlling Conditional Language Models without Catastrophic Forgetting

Machine learning is shifting towards general-purpose pretrained generative models, trained in a self-supervised manner on large amounts of data, which can then be applied to solve a large number of tasks. However, due to their generic training methodology, these models often fail to meet some of the downstream requirements (e.g., hallucinations in abstractive summarization or style violations in code generation). This raises the important question of how to adapt pre-trained generative models to meet all requirements without destroying their general capabilities ("catastrophic forgetting"). Recent work has proposed to solve this problem by representing task-specific requirements through energy-based models (EBMs) and approximating these EBMs using distributional policy gradients (DPG). Despite its effectiveness, this approach is however limited to unconditional distributions. In this paper, we extend DPG to conditional tasks by proposing Conditional DPG (CDPG). We evaluate CDPG on four different control objectives across three tasks (translation, summarization and code generation) and two pretrained models (T5 and GPT-Neo). Our results show that fine-tuning using CDPG robustly moves these pretrained models closer towards meeting control objectives and -- in contrast with baseline approaches -- does not result in catastrophic forgetting.

==> conditional DPG ICML2022/math_commands.tex <==
\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\KLhat}{\hat{D}_{\mathrm{KL}}}
\newcommand{\TVD}{\mathrm{TVD}}
\newcommand{\CE}{\mathrm{CE}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\pit}{{\pi_\theta}}
\newcommand{\nablapitlog}{\nabla_{\theta} \log \pit(x)}
\newcommand{\sprod}[2]{{\left<#1,#2\right>}}


\newcommand\BibTeX{B\textsc{ib}\TeX}
\newcommand{\GDC}{GDC }
\newcommand{\GDCon}{GDC\textsuperscript{on} }
\newcommand{\GDCoff}{GDC\textsuperscript{off} }
\newcommand{\GDCplus}{GDC\texttt{++} }
\newcommand{\DPG}{DPG }
\newcommand{\DPGon}{DPG\textsuperscript{on} }
\newcommand{\DPGoff}{DPG\textsuperscript{off} }

\newcommand{\Ron}{R^\text{ on}_\theta(x)}
\newcommand{\Roff}{R^\text{ off}_\theta(x)}
\newcommand{\Aon}{A^\text{ on}_\theta(x)}
\newcommand{\Aoff}{A^\text{ off}_\theta(x)}
\newcommand{\ARL}{A^\text{ RL}_\theta(x)}
\newcommand{\Bon}{B^\text{on}(x)}
\newcommand{\Boff}{B^\text{off}(x)}
\newcommand{\BRL}{B^\text{RL}(x)}


\newcommand{\grad}{G_\theta}
\newcommand{\gradest}{G(\theta)}
\newcommand{\vargrad}{\mathrm{Var}(\grad)}
\newcommand{\mgrad}{\mathbf{\mu}(\grad)}

\newcommand{\Adv}{\mathrm{A}}
\newcommand{\mAdv}{\mu^\Adv}
\newcommand{\mAbsAdv}{\mu^{|\Adv|}}
\newcommand{\varAdv}{\mathrm{Var}\left(\Adv\right)}

\newcommand{\nabt}{\nabla_\theta}
\newcommand{\Rt}{R_\theta}

\newcommand{\EX}[1]{\E_{#1}}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\newif\ifready
%\readytrue: ready-to-submit version
%\readyfalse: commented version

\readyfalse
%  \readytrue

\ifready
\newcommand{\ftk}[1]{}
\newcommand{\fgk}[1]{}
\newcommand{\fmd}[1]{}
\newcommand{\fhe}[1]{}
\newcommand{\annot}[1]{}
\newcommand{\todo}[1]{}
\newcommand{\ptgk}[1]{{#1}}
\else
\newcommand{\ftk}[1]{}
\newcommand{\fgk}[1]{}
\newcommand{\fmd}[1]{}
\newcommand{\fhe}[1]{}
\newcommand{\ptgk}[1]{\textcolor{orange}{#1}}
% \newcommand{\ftk}[1]{{\color{red}\footnote{\textcolor{red}{TK: #1}}}}
% \newcommand{\fgk}[1]{{\color{orange}\footnote{\textcolor{orange}{GK: #1}}}}
% \newcommand{\fmd}[1]{{\color{blue}\footnote{\textcolor{blue}{MD: #1}}}}
% \newcommand{\fhe}[1]{{\color{olive}\footnote{\textcolor{olive}{HE: #1}}}}
\newcommand{\annot}[1]{\textbf{\textcolor{purple}{#1~}}}
\newcommand{\todo}[1]{\textcolor{red}{#1~}}

\fi

% MD June 2022
% comments relative to final version (fvXX)
\newcommand{\fvmd}[1]{\footnote{\textcolor{blue}{MD: #1}}}


% MD (27 Jan 2022) edit for final version
% \newcommand{\ptmd}[1]{\textcolor{blue}{#1}}
\newcommand{\ptmd}[1]{{#1}}
% 

\newcommand{\Rtheta}{R_\theta}

\newcommand{\NER}{\mathrm{NER}}

==> conditional DPG ICML2022/sections/algorithm_pointwise.tex <==
\begin{algorithm}[H]
\caption{Estimating $\EX{c \sim \tau(c)} \KL(p_c,\pit)$}
\label{algo:kl}
% \begin{small}
\begin{algorithmic}[1]
\Require a distribution over queries $\tau(c)$
\Require conditional model $\pit$
\Require $N$, number of contexts
\Require $M$, number of samples for each context
\State sample batch $\{c_1, ... , c_i, ... , c_N\}$ from $\tau(c)$
\For{$i \in \{1, \dots, N\}$}
    \State sample batch $\{x_1, ... , x_j , ... , x_{M}\}$ from $\pi_\theta(x|c_{i})$
        \State $\hat{Z}_{c_i} = \frac{1}{M} \sum_{j=1}^M \frac{P_{c_i}(x_j)}{\pi_\theta(x_j|c_i)}$
\EndFor 
\State $\KL(p,\pit) = \frac{1}{NM} 
\sum_{i=1}^N \sum_{j=1}^M \Big[\frac{1}{\hat{Z}_{c_i} + \epsilon} \frac{P_{c_i}(x_j)}{\pit(x_j|c_i)} \Big[ -\log \hat{Z}_{c_i} + \log \frac{P_{c_i}(x_j)}{\pit(x_j|c_i)} \Big] \Big]$
\Ensure An estimate of $\EX{c \sim \tau(c)} \KL(p_c,\pit)$
\end{algorithmic}
% \end{small}
\end{algorithm}

==> conditional DPG ICML2022/sections/discussion.tex <==
We presented CDPG, a principled approach to fine-tuning conditional language models to satisfy arbitrary constraints. In contrast with other methods, CDPG does not require ground truth training data and is able to shift model distribution in a minimally invasive way. In consequence, models fine-tuned with CDPG share desired characteristics, such as improved factual consistency or compilability, with the fluency and diversity of the original model.

Future work could evaluate CDPG on other tasks --- such as dialogue --- as well as explore other control objectives such as constraining the semantics (as opposed to syntax) of generated Python functions. Another future direction consists in extending CDPG to approximate conditional analogues of the more general, \emph{exponential-form} \citep{khalifa_2021} EBMs which can represent \emph{distributional} constraints, namely, desired expected values for certain features of generated samples.

==> conditional DPG ICML2022/sections/experiments.tex <==
We evaluate CDPG as well as three baselines on four control objectives across three tasks: translation, summarization and code generation. Each task is associated with $C_\text{train}$, a set of contexts $c$ used for prompting the model: these are English source sentences for translation, Python function signatures in case of code generation and source documents in case of summarization. When computing evaluation metrics, we sample contexts from a held out set $C_\text{test}$ not used for training. In addition to that, for each experiment, we measure $\E_{c\sim\tau(c)} \KL(p_c, \pit)$, the expected forward KL divergence from the optimal distribution $p_c$, as well as $\E_{c\sim\tau(c)} \KL(\pit, a)$, the expected reverse KL divergence from the original pretrained model.\footnote{See Appendix \ref{sec:appendix-metrics} for details of metrics calculations.}.

\subsection{Baselines} 

% \paragraph{Unconditional DPG} We compare our algorithm against the original DPG for unconditional EBMs developed by \cite{A-parshakova-etal-2019-global} and extended by \cite{khalifa_2021}. This algorithm differs from conditional DPG: it ignores the partition function $Z_c$ in the denominator of \eqref{eq:grad-est} assuming it to be constant (which it is for unconditional EBMs but not for conditional ones). For a fair comparison, we use the on-policy variant (called ``DPG-on'' in \citep{opt-rl-arxiv-2019}) where we sample from $\pit$ as opposed to a different proposal distribution $q$. 

\paragraph{DPG-like ablation} We compare our algorithm with an ablation (labeled as ``DPG'' on all figures) that sets $Z_c$ in the denominator of \eqref{eq:grad-est} to a constant $Z$ which is the running mean of $P_c(x)$ across $x$'s and $c$'s. This ablation resembles the original DPG algorithm for unconditional EBMs developed by \citep{A-parshakova-etal-2019-global} and extended by \citep{khalifa_2021}. While the partition function is constant for unconditional EBMs, in conditional EBMs $Z_c$ varies with $c$. Therefore, the DPG-like ablation performs gradient updates using biased gradient estimates.

\paragraph{Reinforcement learning} The problem of fine-tuning a pretrained model to satisfy a pointwise constraint $b(x,c)$ can be posed as maximising tbe expected reward $\EX{c  \sim \tau(c)}\EX{x\sim  \pit(x|c)} R(x,c)$. We consider two instances of this approach: Reinforce \citep{Williams92Reinforce} and Ziegler \citep{Ziegler19}. For Reinforce, we simply define $R(x,c) = b(x,c)$. Ziegler prevents too large departures from $a$ by adding a KL penalty term and defining $R(x,c) = b(x,c) - \beta \KL(\pit, a)$, where $\beta$ is a hyperparameter updated using an adaptive schedule.

\subsection{Translation}
\label{experiments:translation}

\begin{figure*}[h]  
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_MT.pdf} 
    \caption{\small{Translation with terminology constraint. Evaluation metrics: fraction of samples satisfying constraint $b(x)$ ($\uparrow$ better), expected $\KL(p_c,\pit)$ ($\downarrow$ better) and $\KL(\pit,a)$ ($\downarrow$ better), and BLEU-4 score ($\uparrow$ better) for models obtained from fine-tuning with conditional DPG, DPG, Ziegler and Reinforce.}}
    \label{fig:translation}
\end{figure*}


\paragraph{Dataset} For the translation task, $\tau(c)$ from Algorithm \ref{algo:training-loop} is a uniform distribution over a fixed set of English sentences. We sampled 5k English sentences containing numeral nouns from the English-French subcorpus of the Europarl dataset, version 7 \citep{koehn-2005-europarl}. Metrics are computed for generated translations of another set of 5k English sentences from the test split of Europarl. Note that neither CDPG nor the baselines utilise ground truth translations (references); we compute $b(x,c)$ based on source documents and {\it generated} translations. Ground-truth translations are only used for evaluating the BLEU score of generated translations.

\paragraph{Model} We conduct our experiments on the T5 architecture \citep{2020t5}, using the pre-trained model \texttt{t5-small} as $\pit$. During fine-tuning, we generate translations $x$ conditioned on a source sentence $c$ by pure ancestral sampling from $\pit$. For evaluation, we follow the setup described by \cite{2020t5} and use beam search decoding with beam size 4.

\paragraph{Metrics} In addition to measuring  expected $\KL(p_c,\pit)$ and $\KL(\pit,a)$, we evaluate the forgetting of T5's capabilities in terms of BLEU-4 score \cite{10.3115/1073083.1073135}, a measure of translation quality understood as overlap between generated and ground-truth translation.

\paragraph{Constraint} We implement the constraint scorer as table lookup: $b(x,c) = 1$  if for every occurrence of a given numeral noun (e.g. ``two'') in a source sentence $c$, a corresponding digit (``2'') occurs in its translation $x$. Otherwise, $b(x,c) = 0$.

\paragraph{Results}

We present the results of the translation task on Figure \ref{fig:translation}. Initial constraint satisfaction is very low: 0.006. Intuitively, it's very unlikely for T5 to translate ``two'' as ``2'', not as ``deux''. However, CDPG is able to boost that number to 0.7 and reduce the expected divergence from its target distributions $p_c$ almost twofold, outperforming DPG by a wide margin. It also outperforms Reinforce by staying closer to the original distribution $a$ and not suffering from almost any drop in BLEU-4 score. (Note that some drop is necessary for satisfying the constraint, because ground truth translations with respect to which BLEU-4 is computed almost don't satisfy the constraint themselves.) In contrast, Reinforce improves constraints satisfaction only at the cost of heavy divergence from $a$: it learns to append all the digits at the end of each translation, thus ensuring constraint satisfaction (see Appendix \ref{sec:appendix_samples_translation} for sample translations). This is reflected in a catastrophic drop in BLEU-4 score. Ziegler, on the other hand, fails to improve constraint satisfaction and stays \emph{too close} to the original distribution~$a$. 

\subsection{Summarization}

\begin{figure*}[h]  
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_summarization_entities.pdf} 
    \caption{\small{Summarization with factual consistency constraint. Evaluation metrics: expected $\KL(p_c,\pit)$ ($\downarrow$ better) and $\KL(\pit,a)$ ($\downarrow$ better), precision-source ($\uparrow$ better), recall-target ($\uparrow$ better), number of named entities ($\uparrow$ better), Distinct-2 ($\uparrow$ better), ROUGE-L ($\uparrow$ better) for models obtained from fine-tuning with conditional DPG, DPG, Ziegler and Reinforce.}}
    \label{fig:summarization_entities_metrics}
\end{figure*}

% \subsubsection{Experimental setup}

\paragraph{Dataset} To conduct our summarization experiments, we use the CNN/DailyMail dataset \citep{nallapati-etal-2016-abstractive} and sample 5k source documents from the train and test subsets to use for fine-tuning and evaluation, respectively.
%
  We use ground truth summaries only for computing reference-based evaluation metrics such as ROUGE score or recall-target. Ground truth summaries are not used in training.

\paragraph{Model} We use the same model as in the translation task (\texttt{t5-small}). For fine-tuning, we generate summaries $x$ conditioned on a source document $c$ by pure ancestral sampling from $\pit$; for evaluation, we use beam search with beam size 4.

\paragraph{Constraints} Following \cite{nan-etal-2021-entity}, we define an entity-level factual consistency constraint as a product of two constraints: there must be at least four named entities in the summary $x$ and all the named entities $x$ must have occurred in the source $c$. More formally, let $\NER(\cdot)$ denote the set of named entities found in a text and $|\cdot|$ the number of elements of a set. Then, $b(x,c) = 1$ iff $[|\NER(x)| \geq 4] \land [\NER(x) \subseteq \NER(c)]$ and $b(x,c) = 0$ otherwise.

\paragraph{Metrics} In addition to measuring expected $\KL(p_c,\pit)$ and $\KL(\pit,a)$, we evaluate the quality and factual consistency of generated summaries using the following metrics: 
\begin{enumerate}
    \itemsep0em 
    \item Precision-source \citep{nan-etal-2021-entity}, defined as $[|\NER(x) \cap \NER(x)|]/|\NER(x)|$ is the percentage of named entities in the summary that can be found in the source. Low precision-source indicates severe hallucination,
    \item Recall-target \citep{nan-etal-2021-entity}, defined as $[|\NER(x) \cap \NER(x)|]/|\NER(t)|$, is the percentage of named entities in the target summary $t$ that can be found in the generated summary $x$.
    \item Distinct-2 \citep{li-etal-2016-diversity}, a measure of text diversity in terms of the frequency of bigram repetitions within a single continuation $x$,
    \item ROUGE-L \citep{lin-2004-rouge}, a measure of summarization quality in terms of unigram overlap between the source document and ground truth summary.
\end{enumerate}
See Appendix \ref{sec:appendix-code} for on how scorers $b$ and
metrics are computed for summarization experiments.

\paragraph{Results}

We present the evolution of our 7 metrics through time on Figure \ref{fig:summarization_entities_metrics}. CDPG is the only method stably decreasing expected $\KL(p_c,\pit)$ and thus approaching (as opposed to drifting away from) optimal distributions $p_c$. This is reflected in moderate divergence from $a$ and translates into downstream metrics. Summaries generated by the fine-tuned model contain, on average, more named entities. Moreover, name entities in summaries are both more factually consistent with source (an increase in precision-source) and more relevant (an increase in recall-target). The tendency towards mentioning more factually consistent named entities increases the bigram diversity within summaries (Distinct-2) and the overall quality of generated summaries compared to ground truth (ROUGE-L). This last results might seem surprising given that CDPG did \emph{not} have access to ground truth summaries. A plausible explanation is that the original pretrained model was biased towards mentioning too few factually correct entities, at least compared to ground truth summaries. Satisfying the factual consistency constraint reduced this bias.

Baseline approaches fall short of achieving similar results. The DPG-like ablation, the closest contender, still leaves a significant gap in terms of \emph{all} metrics and is far less stable than CDPG (e.g. its $\KL(p_c,\pit)$ starts to diverge again after around 500 epochs). Ziegler stays extremely close to the original model $a$, failing to improve its shortcomings. In contrast, Reinforce heavily departs from $a$ pushing it to mention a large number of named entities. This results in artificially inflated recall-target but no increase in precision-source and a \emph{decrease} in ROUGE-L. The additional named entities frequently are frequently irrelevant (i.e. not mentioned in ground truth summaries) or simply hallucinated. See Tables \ref{tab:sum_0_samples}-\ref{tab:sum_4_samples} in the Appendix for randomly chosen summaries of documents in the test set.

\begin{figure*}[h]  
    \centering
    \begin{subfigure}[t]{\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_code_comp.pdf}
    \caption{\small{Compilability constraint}}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=0.97\linewidth]{figures/ctrlgen_code_pep8.pdf}
    \caption{\small{PEP8 constraint}}
    \end{subfigure}
    \caption{\small{Code generation with compilability (a) and PEP8 (b) constraint. Evaluation metrics: compilability ($\uparrow$ better), number of PEP8 errors ($\downarrow$ better), expected $\KL(p_c,\pit)$ ($\downarrow$ better) and $\KL(\pit,a)$ ($\downarrow$ better),  number of characters, AST node count ($\uparrow$ better) for models obtained from fine-tuning with CDPG, DPG, Ziegler and Reinforce.}}
    \label{fig:code_metrics}
\end{figure*}

\begin{figure*}[h]  
    \centering
    \begin{subfigure}[t]{\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_comp_errors1.pdf}
    \caption{\small{Relative frequencies of compilation errors}}
    \end{subfigure}
    \begin{subfigure}[t]{\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_pep8_errors1.pdf}
    \caption{\small{Absolute frequencies of PEP8 violations}}
    \end{subfigure}
        \begin{subfigure}[t]{\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_ners1.pdf}
    \caption{\small{Absolute frequencies of named entities}}
    \end{subfigure}
    \caption{\small{Relative frequencies of most common compilation errors (a), absolute frequencies of most common PEP8 violations (b) and absolute frequencies of named entities (c) in a batch of 10280 samples from the original model $a$ as well as models obtained from fine-tuning with CDPG, DPG, Ziegler and Reinforce.}}
    \label{fig:errors}
\end{figure*}

\begin{figure*}[h]  
    \centering
    \begin{subfigure}[t]{.24\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_translation_zipf.pdf}
    \caption{\small{Translation with terminology constraint}}
    \end{subfigure}
    \begin{subfigure}[t]{.24\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_summarization_length_zipf.pdf}
    \caption{\small{Summarization with factual consistency constraint}}
    \end{subfigure}
    \begin{subfigure}[t]{.24\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_code_comp_zipf.pdf}
    \caption{\small{Code generation with compilability constraint}}
    \end{subfigure}
    \begin{subfigure}[t]{.24\textwidth}
    \vskip 0pt
    \centering
    \includegraphics[width=\linewidth]{figures/ctrlgen_code_pep8_zipf.pdf}
    \caption{\small{Code generation with PEP8 constraint}}
    \end{subfigure}
    \caption{\small{Token frequency against token rank computed for tokens in 10280 samples from $a$, Conditional DPG and baselines. Longer tails imply more diverse samples.}}
    \label{fig:zipf}
\end{figure*}

\subsection{Code generation}


\paragraph{Dataset}

For code generation experiments, we condition a language model on Python function signatures (both of methods and standalone functions) extracted from the Python150 dataset which consists of Python source code  obtained from GitHub \citep{Raychev2016}. We use the code provided by  \cite{roziere2020unsupervised} for function extraction and randomly choose 5k functions for $C_\text{train}$ and 5k for $C_\text{test}$. $\tau(c)$ is a uniform distribution over these signatures. Note that neither in fine-tuning nor in evaluation do we use ground truth function bodies.

\paragraph{Model} We conduct experiments using GPT-Neo \citep{gpt-neo}: an off-the-shelf, freely available autoregressive language model mirroring the GPT-3 architecture \citep{gpt3}. GPT-Neo's training set included 85 GiB of source code from GitHub which endowed it with some code completion abilities \citep{gao2020pile}. We use the \texttt{gpt-neo-125} variant available on Huggingface Transformers \citep{huggingface}. During both fine-tuning and evaluation we generate function bodies by conditioning on signatures using pure ancestral sampling.
\paragraph{Constraints}

For experiments with compilability control condition, we check compilability of a Python function declaration obtained by concatenating $[c,x]$ and trying to execute it. $b(x,c) = 1$ if the Python interpreter raises an exception and 0 otherwise. See Appendix \ref{sec:appendix-code} for more details.

For experiments with PEP8-compliance control condition, we check whether a function declaration given by $[c,x]$ violates PEP8 \citep{pep8}, the style guide for Python, by running \texttt{pycodestyle}, an off-the-shelf linter (static code analysis tool).\footnote{\url{https://github.com/PyCQA/pycodestyle}} $b(x,c) = 1$ if the number of PEP8 violations found by \texttt{pycodestyle} is 0, otherwise $b(x,c) = 0$.


\paragraph{Metrics}
We evaluate the quality of generated Python functions using the following metrics:
\begin{enumerate}
    \itemsep0em 
    \item PEP8 error count, the average  number of violations of PEP8,
    \item Compilability, the fraction of samples $[c,x]$ that compile,
    \item The average number of characters in $[c,x]$ (after detokenization),
    \item The average number of nodes in an abstract syntax tree (AST) of sequences that compile. Intuitively, this metric indicates the logical (as opposed to surface) complexity of generated programs.
\end{enumerate}
For more details on how scorers $b$ and metrics are implemented, see Appendix \ref{sec:appendix-code}. 


\paragraph{Results}

We present the evolution of metrics through time on Figure \ref{fig:code_metrics}. CDPG was able to increase the fraction of compilable functions from around 40\% to around 65\% and decrease the average number of PEP8 violations. Incidentally, the PEP8 control objective also leads to an increase in compilability because many PEP8 violations are also compilation errors. Here we note similarly to the results of previous experiments that, CDPG and its DPG-like ablation are the only methods actually approaching optimal distributions $p_c$ and diverging moderately from $a$. This allows them to maintain the original statistics of $a$: length and the number of nodes in AST trees of generated functions. In contrast, Reinforce learns to generate shorter functions (having less opportunity for mistakes) and Ziegler produces heavily degenerated samples \citep{degeneration_HoltzmanBDFC20}: syntactically simple functions with severe repetitions. This is reflected in an increase in length and a decrease in AST nodes count. See Tables \ref{tab:code_0_samples}-\ref{tab:code_2_samples} and Tables \ref{tab:code_pep8_0_samples}-\ref{tab:code_pep8_2_samples} for randomly chosen samples from the compilability and PEP8 experiments, respectively.

Note that the performance gap between CDPG and its DPG-like ablation is much closer for code generation (especially with compilability control objective) than for summarization. This can be accounted for by the normalized standard deviation of partition functions $Z_c$ for EBMs $P_c$ in the range of conditional EBMs $\mathcal{P}$ for each control objective. For code generation, this standard deviation is lower meaning that $Z_c$ in \eqref{eq:grad-est} is better approximated by a constant which can be absorbed into the learning rate $\alpha^{(\theta)}$. For summarization, this variance is higher, therefore ignoring the $Z_c$ term incurs higher bias which translates into worse performance. See Appendix \ref{sec:appendix_nstd_zc} for a comparison.
\subsection{Qualitative analysis}

In the previous sections, we showed how CDPG is able to fine-tune a pretrained model $a$ to satisfy certain constraints without destroying $a$'s capabilities. Here we attempt to gain a better understanding of how different fine-tuning approaches affect the distributions of final models. On Figure \ref{fig:errors} we present frequencies of errors (for the code generation task) and named entities (for the summarisation task) obtained from fine-tuned models. While errors and named entities differ significantly in their frequency, CDPG consistently decreases frequencies of these errors and consistently increases the frequencies of all kinds of named entities, including the long tail of rare ones.

To compare lexical diversity of samples obtained from fine-tuned models (for all four tasks), we plot the frequency of each token (the number of times it occurs) and its rank (its index in a sorted list of tokens) in Figure~\ref{fig:zipf}. CDPG and its DPG-like ablation are able to closely match original token frequencies while Ziegler and Reinforce tend to have shorter tails of rare tokens. 

==> conditional DPG ICML2022/sections/intro.tex <==
% \vspace{-15px}
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.98\columnwidth]{figures/diagram2.pdf}}
\vspace{-10px}
\caption{\small{An overview of our algorithm for fine-tuning conditional language models, illustrated on the terminology-constrained translation task (see Section \ref{experiments:translation} for details).}}
\end{center}
\vspace{-30px}
\end{figure}

Pretrained generative models are shifting the landscape of machine learning research and practice. General purpose models such as the GPT family ~\citep{radford2019language,gpt3,gpt-neo}, T5~\citep{2020t5}, CLIP~\citep{radford2021learning} and Codex~\citep{chen2021evaluating} are trained in a self-supervised manner on large amounts of uncurated data and can then be adapted to specific downstream tasks (e.g. generating Python code) or control objectives (e.g. controlling the style of generated code). Frequently, control objectives are motivated by the desire to address the shortcomings of certain pretrained models. These can be due to the uncurated nature of the original training data (e.g. a large portion of Python source code on the Internet violates PEP8 \citep{pep8}, the Python Style Guide) or the difficulty of learning a desired behaviour by purely self-supervised training (e.g. there is not enough training signal to ensure that a model trained on source code always generates compilable code or that a summarization model always produces factually correct summaries).

The practice of adapting and controlling pretrained generative models poses two open problems. The first is that control objectives frequently lack ground truth data that could be used for supervised fine-tuning; in general, we are only given an indicator $b(x)$ of whether a given sample $x$ from the model satisfies a given control objective. Thus, this restriction calls for approaches that can employ this signal such as reinforcement learning (RL) \citep{pasunuru-bansal-2018-multi,Ziegler19}, weighted decoding \citep{ghazvininejad-etal-2017-hafez,learning2write-holtzman-2018,see-etal-2019-makes} or decoding with perturbed activations \citep{plug_and_play_20}. 

The second problem is \emph{catastrophic forgetting}: most approaches to enforcing a control objective result in a dramatic loss of capabilities of the original model beyond the scope of the control objective. Notably, there exists one approach largely avoiding both of these problems \citep{A-parshakova-etal-2019-global,khalifa_2021}:
representing the control objective as an energy-based models (EBM) and approximating that EBM using distributional policy gradients (DPG). 
%
Although this approach shows great improvements in controlling pretrained language models while avoiding catastrophic forgetting~\citep{khalifa_2021}, it is limited to unconditional generation tasks and cannot fine-tune conditional models that are behind the most impactful NLP tasks such as machine translation, summarization or dialogue systems.

In this paper, we present Conditional DPG (CDPG), an extension of DPG that can approximate \emph{conditional} EBMs. A conditional EBM $\mathcal{P}$ defines an unnormalized distribution for each context $c$ (e.g. a source document). Extending the approach of \citet{khalifa_2021} \ptmd{such a conditional EBM  represents} the ideal behaviour of a generative model, given context $c$, as the distribution that incorporates the control objectives while remaining as close as possible to the original distribution to prevent catastrophic forgetting. 
%
%Then, to approximate conditionals EBMs we build unconditional EBMs $P_c$ on the fly for any given context and estimate their normalizing constants $Z_c \doteq \sum_x P_c(x)$ by importance sampling.
This corresponds to defining multiple distributions $p_c$ indexed by % a context 
$c$, \ptmd{where} each %can be represented as an
\ptmd{is the normalization of an unconditional}
%\emph{unconditional} 
EBM $P_c$ following \citet{khalifa_2021}. We then define the training objective for the conditional model based on minimizing the \emph{average} divergence \ptmd{for} each %$P_c$.
\ptmd{$p_c$}.

We demonstrate the effectiveness of CDPG in addressing shortcomings of pretrained generative models by considering three tasks: translation, summarization and code generation; and two corresponding pretrained generative models: T5 \citep{2020t5} and GPT-Neo \citep{gpt-neo}. 

We start by demonstrating the effectiveness of CDPG on a toy control objective for translation: ensuring that numeral nouns (e.g. ``two'') are translated as digits (e.g. ``1'') while other aspects of translation are unchanged. This problem is an simple instance of broader challenge of incorporating prior information in neural translation models. CDPG is able to make samples satisfying the constraint 116 times more likely. 

For summarization, a similar big, unsolved problem is ensuring that summaries are factually faithful to source documents given that summarization models are prone to hallucinating named entities never mentioned in the source \citep{maynez-etal-2020-faithfulness}. We show that a preference for factually faithful summaries (operationalized as entity-level factual consistency \citep{nan-etal-2021-entity}) can be represented by a conditional EBM. Then, we show that using CDPG to fine-tune T5 to approximate this EBM increases the number of correct and relevant named entities in summaries and improves T5's Rouge score. In contrast with RL approaches, CDPG does not degrade the diversity and quality of summaries.

%
For code generation, we consider the task of generating a Python function given its signature (name and arguments). While general-purpose language models can generate idiomatic Python functions \citep{chen2021evaluating,austin2021program}, they may still struggle to learn some desirable properties of generated code. For instance, a Python function generated by GPT-Neo will compile only 40\% of the time and will contain on average 4 violations of PEP8. We show that using CDPG to approximate a conditional EBM expressing corresponding constraints improves both compilability and PEP8-compliance without hurting the diversity of generated Python code or leading to degeneration~\citep{degeneration_HoltzmanBDFC20}.

The contributions of this paper are as follows:
\vspace{-5px}
\begin{enumerate}
    \itemsep0em 
    \item We introduce a formal framework for representing control objectives for \emph{conditional} generative models as \emph{conditional} EBMs while alleviating \emph{catastrophic forgetting},
    \item We design CDPG, an extension of DPG suitable for approximating conditional EBMs,
    \item We evaluate CDPG on three control objectives across three tasks: machine translation with number format constraints, summarization constrained to be factually correct, code generation constrained to generate compilable Python functions and code generation constrained to respect PEP8.
\end{enumerate}

Code accompanying the paper will be available at \url{https://github.com/naver/gdc}.


==> conditional DPG ICML2022/sections/method_distributional.tex <==
\paragraph{Conditional EBMs}

A standard, ``unconditional'' EBM is a function $P$ from a (discrete, i.e. finite or countable) space $X$ to the non-negative reals, such that the partition function $Z \doteq \sum_{x\in X} P(x)$ is strictly positive and finite. We will denote by lowercase $p$ the normalized distribution over $X$ associated with $P$, namely $p(x) \doteq P(x)/Z$. Let's now consider a discrete set $C$ of conditions $c$. Formally, $P(x,c)$, a \emph{conditional} EBM over $C$ is defined as a function from $C$ to the set of unconditional EBMs over $X$, in other words, a function that maps each $c\in C$ to an unconditional EBM $P_c(x)$ over $X$.
\begin{equation}
    P(x,c): c \mapsto P_c(x)
\end{equation}
We denote by $Z_c$ the partition function of $P_c(x)$, namely: $Z_c \doteq \sum_{x\in X} P_c(x)$, and by $p_c(x)$ the normalized version of $P_c(x)$, namely: $p(x|c) \doteq P_c(x)/Z_c$.

\paragraph{Representing constraints as conditional EBMs}

The problem of fine-tuning a foundation model $a(x|c)$ to satisfy a given control objective can be seen as a constraints satisfaction problem: finding a model $p(x|c)$ that meet the demands of the control objective but at the same time stays as close as possible to $a(x|c)$. We represent such an optimal model as a conditional EBM $P(x,c)$. A control objective can be defined in terms of a feature $\phi(x,c)$\ftk{For simplicity of exposition, I assume here we only have one feature. This is how it's currently implemented and all experiments in this paper will have one feature. I tried the general case but soon came close to something called death by notation.} and a corresponding desired expected value (moment constraint) of $\phi(x,c)$: $\bar{\mu} = \EX{x \sim p} \phi(x,c)$. Let us consider a set of contexts $c \in C$. For each $c$, there is a unique model $p_c(x)$ that satisfies a given a moment constraints while having a minimal KL divergence form $a(\cdot|c)$: an I-projection of $a$ onto the manifold of all distributions satisfying that constraint \citep{csizarShields2004}. $p_c$ can be represented as an unconditional EBM $P_c(x)$. As shown by \citep{A-parshakova-etal-2019-global} and \citep{khalifa_2021}, that unconditional EBM has the following exponential family EBM:
\begin{equation} 
    \label{eq:ebm}
    P_c(x) = a(x|c)e^{\lambda_c \phi(x,c)},
\end{equation}
where $\lambda_c$ is a scalar chosen to ensure that feature moment matches its desired value; $\lambda_i$ can be estimated through self-normalized importance sampling \citep{owen_chapter_importance_sampling_2013} and learned through stochastic gradient descent \citep{A-parshakova-etal-2019-global}.

For instance, if $a(x|c)$ is a summarization model and $\phi_i(x,c)$ denotes the number of words in a summary $x$, $p(x|c)$ will be a summarization model generating summaries that are, on average, $\bar{\mu}$ words long. In most cases, we want $\phi(x,c)$ to be a predicate that \emph{all} samples  $x \sim a(x|c)$ satisfy. For instance, we might want all programs generated by a program synthesizer to be compilable. In that case, we can define $\phi(x,c)$ as a binary scorer and set $\bar{\mu} = 1$\ftk{Added these because I felt a motivating example is needed before a reader gets lost in unfamiliar maths}. Following \citet{khalifa_2021}, we call the first, more general constraint a \emph{distributional} constraint whereas the latter, frequent special case a \emph{pointwise} constraint. For pointwise constraints, $P(x,c)$ admits a simpler, product-of-experts \citep{Hinton02}:\footnote{See \citep[Appendix A.2]{khalifa_2021} for a derivation.}
\begin{equation}
    \label{eq:ebm-pointwise}
    P_c(x) \doteq a(x|c)\phi(x,c).
\end{equation}
We use the product-of-experts form for all pointwise constraints because of its numerical stability and fall back to the exponential family form only for distributional constraints.

\paragraph{Approximating conditional EBMs} 

While $p(x|c)$ represents the target condtional model optimally reconciling distance from $a(a|c)$ and the control objective, sampling or MAP decoding for $p(x|c)$ is intractable for two reasons. First, $p(x|c)$ actually represents a potentially infinite collection of unconditional models of the form $p_c(x)$. Second, each of these conditional models still cannot be easily sampled from because they do not admit autoregressive factorization: $\phi(x,c)$ is only defined for the whole sequence $x$.

The second problem was addressed by \cite{opt-rl-arxiv-2019} and \cite{khalifa_2021} who used the distributional policy gradients (DPG) algorithm to approximate unconditional EBMs $p$ using a \emph{new} unconditional model $\pit$ trained to minimize the cross-entropy between $p$ and itself. Unfortunately, DPG is no longer usable for conditional models that should satisfy infinitely many constraints represented the set of conditional EBMs defined by $P(x,c)$.

To address the second problem, we instead try to find a single model $\pit$ approximating $p$ \emph{on average} across contexts. Concretely, we minimize the expected cross-entropy between $\pit$ and multiple $p_c$'s:

\begin{equation}
    \label{eq:objective}
    \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \CE(p(\cdot|c), \pit(\cdot|c)),
\end{equation}
where the expectation is over $\tau(c)$, a uniform distribution over $c \in C$.\ftk{I was wondering whether speaking of a set $C$ isn't confusing here (it may suggest MC-DPG only fine-tunes for a pre-defined set of contexts and does not generalize outside it). Maybe here we should only speak of $\tau(c)$ in abstract, and only introduce $C_\text{train}$ and $C_\text{test}$ later as approximations of  $\tau(c)$?} This gradient of this objective admits the following form:
\begin{align}
    \nabla_\theta \mathcal{L}(\theta) &= \EX{c \sim \tau(c)} \nabla_\theta\CE(p(\cdot|c), \pit(\cdot|c)) \\
    % &= \EX{c \sim \tau(c)} \nabla_\theta \EX{x \sim p(x|c)} -\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x \sim p(x|c)} \nabla_\theta\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} \frac{p(x|c)}{\pit(x|c)}   \nabla_\theta\log \pit(x|c), \\
        &= -\EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} \frac{P(x,c)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c), \\
\end{align}
where the last step is simply importance sampling from $\pit$.\footnote{This last form of the gradients estimate bears some resemblance to policy gradients methods in reinforcement learning \cite{sutton_policy_gradients} with term $P(x,c)/Z_c\pit(x|c)$ playing the role of a pseudoreward. This similarity, however, is fairly superficial: the objective \eqref{eq:objective} that we minimize is expected cross-entropy, not expected (negative) reward.} 

Now, under the expectation of $\tau(c)$ we can partially evaluate the conditional EBM $P(x,c)$ to obtain an unconditional EBM $P_c(x)$ defined in \eqref{eq:ebm}. \ftk{I don't feel I made a very good job explaining that clearly. What confused me is the distinction between conditional EBMs understood as functions and partially evaluated (fixed $c$) conditional EBMs which are actually unconditional EBM.} That gives rise to the following gradient estimate:
\begin{equation}
    \label{eq:grad-est}
    \nabla_\theta \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} a(x|c)\frac{\exp \big( \lambda_c \phi(x,c) \big)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c).
\end{equation}

For pointwise constraints, \eqref{eq:grad-est} can be simplified to
\begin{equation}
    \label{eq:grad-est-pointwise}
    \nabla_\theta \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} a(x|c)\frac{ \phi(x,c)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c).
\end{equation}


We approximate both expectations in \eqref{eq:grad-est} and \eqref{eq:grad-est-pointwise} by sampling. Intuitively, this corresponds to building unconditional EBMs $P_c(\cdot)$ on the fly for each $c \sim \tau(c)$, computing the EBM ``score'' $P_c(x)$ for each sample from the conditional model $x \sim \pit(\cdot|x)$ and then using this score as a ``pseudoreward`` term $P(x,c)/Z_c\pit(x|c)$ in the policy gradient estimate.

\paragraph{Estimating $Z_c$ and $\lambda_c$}

There are two terms in \eqref{eq:grad-est} that remain difficult to evaluate. For a single unconditional EBN, \cite{khalifa_2021} had no need to evaluate its partition function: it just scaled gradient estimates and therefore could be absorbed into the learning rate. In our case, each $Z_c$ needs to be evaluated. Furthermore, for unconditional EBMs there was a single $\lambda$ that could be estimated before we start training $\pit$ allowing to decouple EBM definition and EBM approximation. Here both of these steps are fused as we need to define a new EBM for each $c \in C$.

For each $c$, we compute $Z_c$ and $\lambda_c$ using a batch of $M$ samples $\{x_1, \dots, x_j, \dots x_{M}\}$ from $\pi_\theta(x|c_{i})$. $\lambda_c$ is estimated using self-normalized sampling (see Algorithm \ref{algo:snis}) while $Z_c$ is estimated using importance sampling by reweighting samples $x_j$ by their likelihood according to $\pit(\cdot|c_i)$.

\paragraph{Training loop} We train $\pit$ by stochastic gradient descent using the policy gradient estimate \eqref{eq:grad-est}. At each epoch, we first sample $N$ contexts $c$ and then, for each $c$, $M$ samples $x$ from $\pit(x|c)$. We maintain a buffer $\mathcal{B}$ storing each $(c_i, x_j)$ pair along with their corresponding $\lambda_{c_i}$ and $Z_{c_i}$. For pointwise constraints we don't need to compute and store $\lambda_c$. Finally, we shuffle $\mathcal{B}$ and iterate over it to perform gradient steps using \eqref{eq:grad-est} (or \eqref{eq:grad-est-pointwise} for pointwise constraints) with learning rate $\alpha^{(\theta)}$. The procedure for the general case of distributional constraints summarized by Algorithm \ref{algo:training-loop}. $\alpha^{(\theta)}$, $N$ and $M$ are hyperparameters. Values used for experiments are reported in Tables \ref{table:code-hyperparams}-\ref{table:summarization-hyperparams} in the Appendix.

\begin{algorithm}[H]
\caption{Distributional Conditional DPG using Monte Carlo}
\label{algo:training-loop}
\begin{algorithmic}[1]
\begin{small}
\Require conditional EBM $P(x,c)$, initial model $a(x|c)$, desired moment $\bar{\mu}$
\State $\pi_\theta \gets a$
\For{each iteration}
    \State $\mathcal{B} \leftarrow \{\}$ \Comment{clear buffer}
    \State sample batch $\{c_1, ... , c_i, ... , c_N\}$ from $\tau(c)$
    \For{each $c_i$}
        \State sample batch $\{x_1, ... , x_j , ... , x_{M}\}$ from $\pi_\theta(x|c_{i})$
        \State $\lambda_{c_i} = \text{SNIS}(x_{1:n}, c_i, \bar{\mu})$ \Comment{See Algorithm \ref{algo:snis} in Appendix \ref{sec:appendix-algo}}
        \State $\hat{Z}_{c_i} = \frac{1}{n} \sum_{x_j \in x_{1:n}} \frac{a(x_j|c_i)\; \exp(\lambda_c \phi(x_j, c_i)) }{\pi_\theta(x_j|c_i)}$
        \For{each $x_j$}  \Comment{add samples to buffer}
        \State $\mathcal{B}$ $\stackrel{+}\leftarrow$ $(x_j,c_i,\hat{Z}_{c_i}, \lambda_{c_i})$
        \EndFor
    \EndFor
    \For{$(x,c,\hat{Z_c}, \lambda_c)$ in $\operatorname{shuffle}(\mathcal{B})$}
        \State $\theta \gets \theta + \alpha^{(\theta)} \frac{a(x|c) \exp(\lambda_c \phi(x, c))}{\pit(x|c)(\hat{Z_c} + \epsilon)} \ \nabla_\theta \log \pi_\theta(x|c)$
    \EndFor
\EndFor
\Ensure $\pi_\theta$
\end{small}
\end{algorithmic}
\end{algorithm}


==> conditional DPG ICML2022/sections/method_pointwise.tex <==
\paragraph{Unconditional EBMs}
A standard, ``unconditional'' EBM is a function $P$ from a (discrete, i.e. finite or countable) space $X$ to the non-negative reals, such that the partition function $Z \doteq \sum_{x\in X} P(x)$ is strictly positive and finite. We will denote by lowercase $p$ the normalized distribution over $X$ associated with $P$, namely $p(x) \doteq P(x)/Z$. 
\citet{khalifa_2021} show that the problem of fine-tuning a pretrained model $a(x)$ to satisfy a control condition $b(x)=1 \ \forall x \in X$, where $b(x)$ is a binary scorer for a desired feature, while minimizing the divergence to the original a(x) has a unique solution given by the probability distribution $p$ associated with the EBM

\begin{equation}
    P(x) = a(x)b(x).
\end{equation}

In information-geometric terms, $p$ is \ptmd{the} I-projection of $a$ onto the manifold of all distributions satisfying \ptmd{the} constraint given by $b$~\citep{csizarShields2004}.%
% \fvmd{A less ``pedantic'' explanation in this simple case is that p(x) is just a(x|b(x)=1). What should we say?}

\paragraph{Conditional EBMs}

Let us now consider a discrete, potentially infinite set $C$ of conditions $c$. Formally, $\mathcal{P}$, a \emph{conditional} EBM over $C$, is defined as a function from $C$ to the set of unconditional EBMs over $X$, in other words, a function that maps each $c\in C$ to an unconditional EBM $P_c$ over $X$:
% \vspace{-5px}
\begin{align}
    \mathcal{P} &: c \mapsto P_c, \\
    P_c &: x \mapsto \mathbb{R}_{+}.
\end{align}
We denote by $Z_c$ the partition function of $P_c(x)$, namely: $Z_c \doteq \sum_{x\in X} P_c(x)$, and by $p_c(x)$ the normalized version of $P_c(x)$, namely: $p_c(x) \doteq P_c(x)/Z_c$.%
%%%%%
% \fmd{I am not fully sure of what is your intention relative to the notation $P(x,c)$, but I think a better notation would be to use, say, bold $\bm{P}$ for the ``conditional model'', and to define $\bm{P}$ as a \emph{function} from $C$ to the set of unconditional EBMs over $X$, namely $\bm{P}: c \rightarrow P_c$, where $P_c$ is an unconditional EBM, namely a function from $X$ to the reals. An alternate notation for $\bm{P}$ might be $P_C$. \textcolor{red}{Isn't $P(x,c)$ the function you describe?}}
%%%%%
% We will use the shortcut notation $\mathcal{P}(x|c)$ to denote $\mathcal{P}(c)(x)$: a conditional EBM $\mathcal{P}$ evaluated first at a given context $c$ (resulting in an unconditional EBM $P_c$) and then at given $x$ (resulting in a non-negative EBM score).

\paragraph{Representing constraints as conditional EBMs}

The problem of fine-tuning a pretrained model $a(x|c)$ to satisfy a control objective (e.g. generating factually correct summaries) can be seen as a constraint satisfaction problem: finding a model $p_c(x)$ that meets the demands of the control objective but at the same time stays as close as possible to the original pretrained model $a(x|c)$. We represent such an optimal model as an unconditional EBM $P_c(x)$. A control objective can be defined in terms of a
binary scorer $b(x,c)$ such that $b(x,c) = 1$ if a sample $(c,x)$ satisfies a constraint given by a control objective (e.g. $x$ is factually correct with respect to $c$) and $b(x,c) = 0$ otherwise. Let us consider a set of contexts $C$. For each $c \in C$, we can frame the problem of finding the unique model $p_c(x)$ such that (i) $b(x,c) = 1$  for all samples $x \sim p_c(x)$, and (ii) $p_c(\cdot)$ has minimal KL divergence from $a(\cdot|c)$ as an instance of the unconditional case already considered by \citet{khalifa_2021}. Following our example, $p_c$ could be a distribution over factually correct summaries of $c$ as similar as possible to a distribution over summaries which the original model $a$ would produce for a document $c$. Therefore, $p_c$ can be represented as an unconditional EBM $P_c(x)$ of the following form:\footnote{\citet{khalifa_2021} provide a more general, exponential family form of this EBM. The product-of-experts \citep{Hinton02} form in \eqref{eq:ebm} is a special case of the exponential form, see \citep[Appendix A.2]{khalifa_2021}.}
\begin{equation} 
    \label{eq:ebm}
    P_c(x) \doteq a(x|c)b(x,c).
\end{equation}%
\vspace{-10px}
\paragraph{Approximating conditional EBMs} 

While $\mathcal{P}$ represents the target conditional model optimally reconciling distance from $a(x|c)$ and the control objective, sampling and MAP decoding for
\ptmd{$\mathcal{P}$} 
%$p(x|c)$ 
is intractable for two reasons. First, \ptmd{$\mathcal{P}$} actually represents a potentially infinite collection of unconditional models of the form $p_c(\cdot)$. Second, each of these unconditional models still cannot be easily sampled from because they do not admit an autoregressive factorisation: $b(x,c)$ is only defined for the whole sequence $x$.

The second problem was addressed by \cite{opt-rl-arxiv-2019}
and \cite{khalifa_2021} who used the distributional policy gradients (DPG) algorithm to approximate unconditional EBMs $p$ using a \emph{new} unconditional model $\pit$ trained to minimize the cross-entropy $\CE(p,\pit)$. 
Unfortunately, DPG is not directly usable for a conditional model covering many contexts $c$.
% no longer usable for conditional models that should satisfy infinitely many constraints represented by the set of conditional EBMs defined by $\mathcal{P}$.
% Unfortunately, DPG is no longer usable for conditional models $\mathcal{P}$ that cover many constraints $c$ and models $P_c$"

To address these problems, we instead try to find a \emph{single} \ptmd{seq2seq} model $\pit$ approximating $p$ \emph{on average} across contexts. Concretely, we minimize the expected cross-entropy between $\pit$ and multiple $p_c$'s:
\vspace{-5px}
\begin{equation}
    \label{eq:objective}
    \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \CE(p_c(\cdot), \pit(\cdot|c)),
\end{equation}
where the expectation is over $\tau(c)$, a distribution over $c \in C$.%
%%%%%
\ftk{I was wondering whether speaking of a set $C$ isn't confusing here (it may suggest MC-DPG only fine-tunes for a pre-defined set of contexts and does not generalize outside it). Maybe here we should only speak of $\tau(c)$ in abstract, and only introduce $C_\text{train}$ and $C_\text{test}$ later as approximations of  $\tau(c)$?
\textcolor{blue}{MD: IMO, $\tau$ is \emph{not} uniform over $C$, and could be over an infinite set of conditions. The loss $\mathcal{L}$, if you want, is the true average loss that would be incurred by a user at test time. Ideally, training should then indeed draw $c$ according to the same distribution. It is only for (not fully convincing to me) practical reasons that the training is limited to a few $c$'s. Actually, my impression is that, even with the MC approach to estimating $Z_c$, you could actually draw $c$ according to $\tau$ during training, and sample \emph{two} $x$'s for this $c$; just sampling one $x$ would not work with the MC estimate for $Z_c$, but two might work (I am not sure, just a hunch). I think part of the confusion comes from wanting to impose that training $c$'s and test $c$'s be disjoint, which is contrary to general ML principles. Of course, if because of practical (artificial ?) considerations, you limit the $c$'s used at training time to a small set, it may be more convincing then to ensure that elements of your test set were not seen at training time, but this is a different point.
}} 
%%%%%
The gradient of this objective takes the following form:
\begin{align}
    \nabla_\theta \mathcal{L}(\theta) &= \EX{c \sim \tau(c)} \nabla_\theta\CE(p_c(\cdot), \pit(\cdot|c)) \\
    % &= \EX{c \sim \tau(c)} \nabla_\theta \EX{x \sim p(x|c)} -\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x \sim p_c(x)} \nabla_\theta\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} \frac{p_c(x)}{\pit(x|c)}   \nabla_\theta\log \pit(x|c), \label{eq:importance-sampling}\\
    &= -\EX{c \sim \tau(c)} \EX{x \sim \pit(x|c)} \frac{P_c(x)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c), \label{eq:grad-est} 
\end{align}
where in \eqref{eq:importance-sampling} we applied importance sampling from $\pit$ and \eqref{eq:grad-est} expresses $p_c$ in terms of unconditional EBM $P_c$ and its  partition function $Z_c$.\footnote{This last form of the gradients estimate bears some resemblance to policy gradients methods in reinforcement learning \citep{sutton_policy_gradients} with term $P_c(x)/Z_c\pit(x|c)$ playing the role of a pseudoreward. This similarity, however, is fairly superficial: our minimization objective \eqref{eq:objective} is expected cross-entropy (over contexts), not expected (negative) reward. See \cite{RMvsDM} for extended discussion.} 

We approximate both expectations in \eqref{eq:grad-est} by sampling.
%%%%
\ftk{I don't feel I made a very good job explaining that clearly. What confused me is the distinction between conditional EBMs understood as functions and partially evaluated (fixed $c$) conditional EBMs which are actually unconditional EBM. \textcolor{blue}{MD: yes, I think it would be much clearer to consider conditional EBMs as functions, as I have noted above. Basically, I was trying to introduce a notation $\bm{P}$ for what in lambda calculus would be denoted by $\lambda c \lambda x\ P(c,x)$.}} 
%%%%%
Intuitively, this corresponds to building unconditional EBMs $P_c(\cdot)$ on the fly for each $c \sim \tau(c)$, computing the EBM ``score'' $P_c(x)$ for each sample from the \ptmd{seq2seq model $x \sim \pit(\cdot|c)$} and then using this score as a ``pseudoreward`` term $P_c(x)/(Z_c\pit(x|c))$ in the policy gradient estimate.

\begin{algorithm}[H]
\caption{Conditional DPG (CDPG)}
\label{algo:training-loop}
\begin{algorithmic}
\begin{small}
\Require conditional EBM $P_c(x)$, initial model $a(x|c)$
\State $\pi_\theta \gets a$
\For{each iteration}
    \State $\mathcal{B} \leftarrow \{\}$ 
    \State sample batch $\{c_1, ... , c_i, ... , c_N\}$ from $\tau(c)$
    \For{each $c_i$}
        \State sample batch $\{x_1, ... , x_j , ... , x_{M}\}$ from $\pi_\theta(x|c_{i})$
        \State $\hat{Z}_{c_i} = \frac{1}{M} \sum_{j=1}^M \frac{P_{c_i}(x_j)}{\pi_\theta(x_j|c_i)}$
        \For{each $x_j$}
            \State $\mathcal{B}$ $\stackrel{+}\leftarrow$ $(x_j,c_i,\hat{Z}_{c_i})$
        \EndFor
    \EndFor
    \For{$(x,c,\hat{Z_c})$ in $\operatorname{shuffle}(\mathcal{B})$}
        \State $\theta \gets \theta + \alpha^{(\theta)} \frac{1}{\hat{Z_c} + \epsilon}\frac{P_c(x)}{\pit(x|c)} \ \nabla_\theta \log \pi_\theta(x|c)$
    \EndFor
\EndFor
\Ensure $\pi_\theta$
\end{small}
\end{algorithmic}
\end{algorithm}

\paragraph{Estimating $Z_c$}

The one term in \eqref{eq:grad-est} that remains difficult to evaluate is the partition function $Z_c$. For a single unconditional EBM, the \citep{khalifa_2021} approach had no need to evaluate the partition function $Z$ as it just scaled gradient estimates and therefore, $Z$ could be absorbed into the learning rate. In the conditional case, $Z_c$ varies with $c$. Therefore for each $c$, we compute $Z_c$ using a batch of $M$ samples $\{x_1, \dots, x_j, \dots x_{M}\}$ from $\pi_\theta(x|c_{i})$. Then, $Z_c$ is estimated using importance sampling by reweighting samples $x_j$ by their likelihood according to $\pit(\cdot|c_i)$.

\paragraph{Training loop} We train $\pit$ by stochastic gradient descent using the gradient estimate \eqref{eq:grad-est}. At each epoch, we first sample $N$ contexts $c$ and then, for each $c$, $M$ samples $x$ from $\pit(x|c)$. We maintain a buffer $\mathcal{B}$ storing each $(c_i, x_j)$ pair along with its corresponding partition function $Z_{c_i}$. Finally, we shuffle $\mathcal{B}$ and iterate over it to perform gradient steps using \eqref{eq:grad-est} with learning rate $\alpha^{(\theta)}$. The procedure is summarized in Algorithm \ref{algo:training-loop}. $\alpha^{(\theta)}$, $N$ and $M$ are hyperparameters. Values used in experiments are reported in Tables \ref{table:code-hyperparams}-\ref{table:summarization-hyperparams} in the Appendix.



==> sections/method_distributional.tex <==
\paragraph{Conditional EBMs}

A standard, ``unconditional'' EBM is a function $P$ from a (discrete, i.e. finite or countable) space $X$ to the non-negative reals, such that the partition function $Z \doteq \sum_{x\in X} P(x)$ is strictly positive and finite. We will denote by lowercase $p$ the normalized distribution over $X$ associated with $P$, namely $p(x) \doteq P(x)/Z$. Let's now consider a discrete set $C$ of conditions $c$. Formally, $P(x,c)$, a \emph{conditional} EBM over $C$ is defined as a function from $C$ to the set of unconditional EBMs over $X$, in other words, a function that maps each $c\in C$ to an unconditional EBM $P_c(x)$ over $X$.
\begin{equation}
    P(x,c): c \mapsto P_c(x)
\end{equation}
We denote by $Z_c$ the partition function of $P_c(x)$, namely: $Z_c \doteq \sum_{x\in X} P_c(x)$, and by $p_c(x)$ the normalized version of $P_c(x)$, namely: $p(x|c) \doteq P_c(x)/Z_c$.

\paragraph{Representing constraints as conditional EBMs}

The problem of fine-tuning a foundation model $a(x|c)$ to satisfy a given control objective can be seen as a constraints satisfaction problem: finding a model $p(x|c)$ that meet the demands of the control objective but at the same time stays as close as possible to $a(x|c)$. We represent such an optimal model as a conditional EBM $P(x,c)$. A control objective can be defined in terms of a feature $\phi(x,c)$\ftk{For simplicity of exposition, I assume here we only have one feature. This is how it's currently implemented and all experiments in this paper will have one feature. I tried the general case but soon came close to something called death by notation.} and a corresponding desired expected value (moment constraint) of $\phi(x,c)$: $\bar{\mu} = \EX{x \sim p} \phi(x,c)$. Let us consider a set of contexts $c \in C$. For each $c$, there is a unique model $p_c(x)$ that satisfies a given a moment constraints while having a minimal KL divergence form $a(\cdot|c)$: an I-projection of $a$ onto the manifold of all distributions satisfying that constraint \citep{csizarShields2004}. $p_c$ can be represented as an unconditional EBM $P_c(x)$. As shown by \citep{A-parshakova-etal-2019-global} and \citep{khalifa_2021}, that unconditional EBM has the following exponential family EBM:
\begin{equation} 
    \label{eq:ebm}
    P_c(x) = a(x|c)e^{\lambda_c \phi(x,c)},
\end{equation}
where $\lambda_c$ is a scalar chosen to ensure that feature moment matches its desired value; $\lambda_i$ can be estimated through self-normalized importance sampling \citep{owen_chapter_importance_sampling_2013} and learned through stochastic gradient descent \citep{A-parshakova-etal-2019-global}.

For instance, if $a(x|c)$ is a summarization model and $\phi_i(x,c)$ denotes the number of words in a summary $x$, $p(x|c)$ will be a summarization model generating summaries that are, on average, $\bar{\mu}$ words long. In most cases, we want $\phi(x,c)$ to be a predicate that \emph{all} samples  $x \sim a(x|c)$ satisfy. For instance, we might want all programs generated by a program synthesizer to be compilable. In that case, we can define $\phi(x,c)$ as a binary scorer and set $\bar{\mu} = 1$\ftk{Added these because I felt a motivating example is needed before a reader gets lost in unfamiliar maths}. Following \citet{khalifa_2021}, we call the first, more general constraint a \emph{distributional} constraint whereas the latter, frequent special case a \emph{pointwise} constraint. For pointwise constraints, $P(x,c)$ admits a simpler, product-of-experts \citep{Hinton02}:\footnote{See \citep[Appendix A.2]{khalifa_2021} for a derivation.}
\begin{equation}
    \label{eq:ebm-pointwise}
    P_c(x) \doteq a(x|c)\phi(x,c).
\end{equation}
We use the product-of-experts form for all pointwise constraints because of its numerical stability and fall back to the exponential family form only for distributional constraints.

\paragraph{Approximating conditional EBMs} 

While $p(x|c)$ represents the target condtional model optimally reconciling distance from $a(a|c)$ and the control objective, sampling or MAP decoding for $p(x|c)$ is intractable for two reasons. First, $p(x|c)$ actually represents a potentially infinite collection of unconditional models of the form $p_c(x)$. Second, each of these conditional models still cannot be easily sampled from because they do not admit autoregressive factorization: $\phi(x,c)$ is only defined for the whole sequence $x$.

The second problem was addressed by \cite{opt-rl-arxiv-2019} and \cite{khalifa_2021} who used the distributional policy gradients (DPG) algorithm to approximate unconditional EBMs $p$ using a \emph{new} unconditional model $\pit$ trained to minimize the cross-entropy between $p$ and itself. Unfortunately, DPG is no longer usable for conditional models that should satisfy infinitely many constraints represented the set of conditional EBMs defined by $P(x,c)$.

To address the second problem, we instead try to find a single model $\pit$ approximating $p$ \emph{on average} across contexts. Concretely, we minimize the expected cross-entropy between $\pit$ and multiple $p_c$'s:

\begin{equation}
    \label{eq:objective}
    \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \CE(p(\cdot|c), \pit(\cdot|c)),
\end{equation}
where the expectation is over $\tau(c)$, a uniform distribution over $c \in C$.\ftk{I was wondering whether speaking of a set $C$ isn't confusing here (it may suggest MC-DPG only fine-tunes for a pre-defined set of contexts and does not generalize outside it). Maybe here we should only speak of $\tau(c)$ in abstract, and only introduce $C_\text{train}$ and $C_\text{test}$ later as approximations of  $\tau(c)$?} This gradient of this objective admits the following form:
\begin{align}
    \nabla_\theta \mathcal{L}(\theta) &= \EX{c \sim \tau(c)} \nabla_\theta\CE(p(\cdot|c), \pit(\cdot|c)) \\
    % &= \EX{c \sim \tau(c)} \nabla_\theta \EX{x \sim p(x|c)} -\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x \sim p(x|c)} \nabla_\theta\log \pit(x|c) \\
    &= -\EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} \frac{p(x|c)}{\pit(x|c)}   \nabla_\theta\log \pit(x|c), \\
        &= -\EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} \frac{P(x,c)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c), \\
\end{align}
where the last step is simply importance sampling from $\pit$.\footnote{This last form of the gradients estimate bears some resemblance to policy gradients methods in reinforcement learning \cite{sutton_policy_gradients} with term $P(x,c)/Z_c\pit(x|c)$ playing the role of a pseudoreward. This similarity, however, is fairly superficial: the objective \eqref{eq:objective} that we minimize is expected cross-entropy, not expected (negative) reward.} 

Now, under the expectation of $\tau(c)$ we can partially evaluate the conditional EBM $P(x,c)$ to obtain an unconditional EBM $P_c(x)$ defined in \eqref{eq:ebm}. \ftk{I don't feel I made a very good job explaining that clearly. What confused me is the distinction between conditional EBMs understood as functions and partially evaluated (fixed $c$) conditional EBMs which are actually unconditional EBM.} That gives rise to the following gradient estimate:
\begin{equation}
    \label{eq:grad-est}
    \nabla_\theta \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} a(x|c)\frac{\exp \big( \lambda_c \phi(x,c) \big)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c).
\end{equation}

For pointwise constraints, \eqref{eq:grad-est} can be simplified to
\begin{equation}
    \label{eq:grad-est-pointwise}
    \nabla_\theta \mathcal{L}(\theta) = \EX{c \sim \tau(c)} \EX{x  \sim \pit(x|c)} a(x|c)\frac{ \phi(x,c)}{Z_c\pit(x|c)}   \nabla_\theta\log \pit(x|c).
\end{equation}


We approximate both expectations in \eqref{eq:grad-est} and \eqref{eq:grad-est-pointwise} by sampling. Intuitively, this corresponds to building unconditional EBMs $P_c(\cdot)$ on the fly for each $c \sim \tau(c)$, computing the EBM ``score'' $P_c(x)$ for each sample from the conditional model $x \sim \pit(\cdot|x)$ and then using this score as a ``pseudoreward`` term $P(x,c)/Z_c\pit(x|c)$ in the policy gradient estimate.

\paragraph{Estimating $Z_c$ and $\lambda_c$}

There are two terms in \eqref{eq:grad-est} that remain difficult to evaluate. For a single unconditional EBN, \cite{khalifa_2021} had no need to evaluate its partition function: it just scaled gradient estimates and therefore could be absorbed into the learning rate. In our case, each $Z_c$ needs to be evaluated. Furthermore, for unconditional EBMs there was a single $\lambda$ that could be estimated before we start training $\pit$ allowing to decouple EBM definition and EBM approximation. Here both of these steps are fused as we need to define a new EBM for each $c \in C$.

For each $c$, we compute $Z_c$ and $\lambda_c$ using a batch of $M$ samples $\{x_1, \dots, x_j, \dots x_{M}\}$ from $\pi_\theta(x|c_{i})$. $\lambda_c$ is estimated using self-normalized sampling (see Algorithm \ref{algo:snis}) while $Z_c$ is estimated using importance sampling by reweighting samples $x_j$ by their likelihood according to $\pit(\cdot|c_i)$.

\paragraph{Training loop} We train $\pit$ by stochastic gradient descent using the policy gradient estimate \eqref{eq:grad-est}. At each epoch, we first sample $N$ contexts $c$ and then, for each $c$, $M$ samples $x$ from $\pit(x|c)$. We maintain a buffer $\mathcal{B}$ storing each $(c_i, x_j)$ pair along with their corresponding $\lambda_{c_i}$ and $Z_{c_i}$. For pointwise constraints we don't need to compute and store $\lambda_c$. Finally, we shuffle $\mathcal{B}$ and iterate over it to perform gradient steps using \eqref{eq:grad-est} (or \eqref{eq:grad-est-pointwise} for pointwise constraints) with learning rate $\alpha^{(\theta)}$. The procedure for the general case of distributional constraints summarized by Algorithm \ref{algo:training-loop}. $\alpha^{(\theta)}$, $N$ and $M$ are hyperparameters. Values used for experiments are reported in Tables \ref{table:code-hyperparams}-\ref{table:summarization-hyperparams} in the Appendix.

\begin{algorithm}[H]
\caption{Distributional Conditional DPG using Monte Carlo}
\label{algo:training-loop}
\begin{algorithmic}[1]
\begin{small}
\Require conditional EBM $P(x,c)$, initial model $a(x|c)$, desired moment $\bar{\mu}$
\State $\pi_\theta \gets a$
\For{each iteration}
    \State $\mathcal{B} \leftarrow \{\}$ \Comment{clear buffer}
    \State sample batch $\{c_1, ... , c_i, ... , c_N\}$ from $\tau(c)$
    \For{each $c_i$}
        \State sample batch $\{x_1, ... , x_j , ... , x_{M}\}$ from $\pi_\theta(x|c_{i})$
        \State $\lambda_{c_i} = \text{SNIS}(x_{1:n}, c_i, \bar{\mu})$ \Comment{See Algorithm \ref{algo:snis} in Appendix \ref{sec:appendix-algo}}
        \State $\hat{Z}_{c_i} = \frac{1}{n} \sum_{x_j \in x_{1:n}} \frac{a(x_j|c_i)\; \exp(\lambda_c \phi(x_j, c_i)) }{\pi_\theta(x_j|c_i)}$
        \For{each $x_j$}  \Comment{add samples to buffer}
        \State $\mathcal{B}$ $\stackrel{+}\leftarrow$ $(x_j,c_i,\hat{Z}_{c_i}, \lambda_{c_i})$
        \EndFor
    \EndFor
    \For{$(x,c,\hat{Z_c}, \lambda_c)$ in $\operatorname{shuffle}(\mathcal{B})$}
        \State $\theta \gets \theta + \alpha^{(\theta)} \frac{a(x|c) \exp(\lambda_c \phi(x, c))}{\pit(x|c)(\hat{Z_c} + \epsilon)} \ \nabla_\theta \log \pi_\theta(x|c)$
    \EndFor
\EndFor
\Ensure $\pi_\theta$
\end{small}
\end{algorithmic}
\end{algorithm}

